Understanding Dataset Difficulty with $\mathcal{V}$-Usable Information

Estimating the difficulty of a dataset typically involves comparing state-of-the-art models to humans; the bigger the performance gap, the harder the dataset is said to be. However, this comparison provides little understanding of how difficult each instance in a given distribution is, or what attributes make the dataset difficult for a given model. To address these questions, we frame dataset difficulty -- w.r.t. a model $\mathcal{V}$ -- as the lack of $\mathcal{V}$-$\textit{usable information}$ (Xu et al., 2019), where a lower value indicates a more difficult dataset for $\mathcal{V}$. We further introduce $\textit{pointwise $\mathcal{V}$-information}$ (PVI) for measuring the difficulty of individual instances w.r.t. a given distribution. While standard evaluation metrics typically only compare different models for the same dataset, $\mathcal{V}$-$\textit{usable information}$ and PVI also permit the converse: for a given model $\mathcal{V}$, we can compare different datasets, as well as different instances/slices of the same dataset. Furthermore, our framework allows for the interpretability of different input attributes via transformations of the input, which we use to discover annotation artefacts in widely-used NLP benchmarks.

==> tables/tab_inter_corr.tex <==

\begin{table}[t]
    \centering
    \small
    
    \begin{tabularx}{\columnwidth}{Xrrrr}
    \toprule
    \multicolumn{5}{c}{SNLI} \\
    \midrule
    {} &  DistilBERT &      GPT2 &  BERT &  BART \\
    \midrule
    DistilBERT &                    1.000 &  0.821 &            0.846 &               0.815 \\
GPT2                    &                    0.821 &  1.000 &            0.809 &               0.822 \\
BERT        &                    0.846 &  0.809 &            1.000 &               0.832 \\
BART      &                    0.815 &  0.822 &            0.832 &               1.000 \\
    \bottomrule
    \end{tabularx}
    
    
     \begin{tabularx}{\columnwidth}{Xrrrr}
    \toprule
    \multicolumn{5}{c}{CoLA} \\
    \midrule
    {} &  DistilBERT &      GPT2 &  BERT &  BART \\
    \midrule
    DistilBERT &                    1.000 &  0.466 &            0.629 &               0.521 \\
GPT2                    &                    0.466 &  1.000 &            0.322 &               0.416 \\
BERT         &                    0.629 &  0.322 &            1.000 &               0.446 \\
BART      &                    0.521 &  0.416 &            0.446 &               1.000 \\
    \bottomrule
    \end{tabularx}
    
    
    
    
    
    
    \caption{
    Cross-model Pearson's $r$ between \pvi estimates made by different finetuned models, on the SNLI and CoLA test sets. 
    For SNLI, the estimates are consistent: what one model finds difficult, others find difficult as well. 
    Since CoLA has less usable information for all these models, the correlations are lower.
    All correlations are highly statistically significant ($p < 0.001$).
    % If a dataset had no usable information, we would expect the correlation to be close to zero.
    % \swabha{is it fair to say that all Transformer based models find similar examples difficult, for most part?} \kawin{probably, but impossible to be certain}
    % \kawin{heatmap takes up too much space}
    % \swabha{nit: best seen as a diagonal, perhaps boldface the largest values that are not 1.0?}
    % \longtermtodos{try similar correlations between fully trained models.}
    }
    \label{tab:inter_corr}
\end{table}

